Repairing Databases over Metric Spaces with Coincidence Constraints

Datasets often contain values that naturally reside in a metric space: numbers, strings, geographical locations, machine-learned embeddings in a Euclidean space, and so on. We study the computational complexity of repairing inconsistent databases that violate integrity constraints, where the database values belong to an underlying metric space. The goal is to update the database values to retain consistency while minimizing the total distance between the original values and the repaired ones. We consider what we refer to as \emph{coincidence constraints}, which include key constraints, inclusion, foreign keys, and generally any restriction on the relationship between the numbers of cells of different labels (attributes) coinciding in a single value, for a fixed attribute set. We begin by showing that the problem is APX-hard for general metric spaces. We then present an algorithm solving the problem optimally for tree metrics, which generalize both the line metric (i.e., where repaired values are numbers) and the discrete metric (i.e., where we simply count the number of changed values). Combining our algorithm for tree metrics and a classic result on probabilistic tree embeddings, we design a (high probability) logarithmic-ratio approximation for general metrics. We also study the variant of the problem where each individual value's allowed change is limited. In this variant, it is already NP-complete to decide the existence of any legal repair for a general metric, and we present a polynomial-time repairing algorithm for the case of a line metric.

==> discrete.tex <==
\subsection{The Discrete Metric}
The following theorem states that for $\costnum$ (i.e., the number of changed cells), there is a linear-time algorithm for a single UID. Note that the theorem applies to any metric space, which is expected as the metric is irrelevant to $\costnum$ (and in particular, we can always translate the problem to the line domain).
\begin{theorem}\label{thm:num-P}
    Suppose that $\Gamma$ consists of a single UID. Given an inconsistent database $D$, an optimal repair of $D$ on $\costnum$ can be computed in linear time.
\end{theorem}
\begin{proof}
  We assume that the UID is $A\sqsubseteq B$. We fix as input an inconsistent database $D$. 
%Let $\vals(D[A])=\set{\alpha_1,\dots,\alpha_n}$ 
%and $\vals(D[B])=\set{\beta_1,\dots,\beta_m}$.
Let $E$ be a repair of $D$. We claim that it suffices to know the set $I(D,E)\defeq\vals(D[A])\cap\vals(D[E])$. Indeed, given $I(D,E)$, we can construct as follows a repair $E'$ such that $I(D,E)=I(D,E')$ and $\costnum(D,E')\leq\costnum(D,E)$:
\begin{enumerate}
    \item For every value $a\in I(D,E)$ with at least one $B$-cell in $D$, we select arbitrary such $B$-cell to be left intact.
    \item For every value $a\in I(D,E)$ with no $B$-cells in $D$, we pick a distinct $B$-cell of $D$ that is not among the ones chosen in the previous step and update its value to $a$.
     \item For every value $a\in\vals(D[A])\setminus I(D,E)$, we change the value of every cell in $D[A]^{-1}(a)$ to that of an arbitrary value of some $B$-cell that we have left in the end.
\end{enumerate}
Note the following. First, we have enough cells to cover the needs of Item~2, since $E$ is a valid solution (hence, $I(D,B)$ is at most the number of $B$-cells of $D$). Second, every updated cell (in steps~1 and~2) is necessarily also updated in $E$, since $E$ is consistent; hence, $\costnum(D,E')\leq\costnum(D,E)$ as claimed. Third, the cost of $E'$ is the cardinality
$|I(D,E)\setminus \vals(D[B]) |$ plus all
cardinalities  $|D[A]^{-1}(a)|$ for every $a\in\vals(D[A])\setminus I(D,E)$.

Henceforth, our algorithm seeks a set $I$ of $M$ or fewer values from $D[A]$, where $M=|\cells(D[B])|$, so that we minimize the cost of $E'$ defined above:
\begin{equation}\label{eq:costP}
\mbox{cost}(I)\defeq\left(\sum_{a\in \vals(D[A])\setminus I} |D[A]^{-1}(a)|\right)+|I\setminus\vals(D[B])|.
\end{equation}
We can also write \cref{eq:costP} as follows.
\begin{equation}\label{eq:num-sep}
\mbox{cost}(I)=
\left(\sum_{a\in \vals(D[A])}|D[A]^{-1}(a)|\right)-
\left(\sum_{a\in I}\gamma(a)\right),
\end{equation}
where:
\[
\gamma(a)=
\begin{cases}
|D[A]^{-1}(a)| & \mbox{if $D[B]^{-1}(a)\neq\emptyset$;} \\
|D[A]^{-1}(a)|-1 & \mbox{otherwise.}
\end{cases}
\]
So, it suffices to find a subset $I$ of $\vals(D[A])$ that maximizes the sum of $\gamma(a)$. Note that the size of $I$ should be at most the number of $B$-cells of $D$. Hence, we select as $I$ the top $\min(|\vals(D[A])|,|\cells(D[B])|)$ values $a$, sorted by descending $\gamma(a)$. 
\end{proof}

The next theorem states that, for a general set of UIDs, finding an optimal repair of $D$ on $\costnum$ is Fixed-Parameter Tractable (FPT), where the parameter is the size of $\Gamma$.

\begin{theorem}\label{thm:num-P}
    Let $\Gamma$ be a set of UIDs. Given an inconsistent database $D$, computing an optimal repair of $D$ on $\costnum$ is FPT for the parameter $|\Gamma|$.
\end{theorem}
\begin{proof}
    TBD
\end{proof}

\eat{
We will construct by dynamic programming a function $\pi: [n]\times[M]\rightarrow\naturals$ so that, in the end, $\pi[q,\ell]$ is the least cost of a any set $P\subseteq\set{\alpha_1,\dots,\alpha_q}$ of $\ell$ $B$-points, 
according to \cref{eq:costP},
where the sum goes from $i=1$ to $i=q$ (hence, we account for only $\alpha_1,\dots,\alpha_q$). In the end, the optimal $P$ is the one that realizes the minimal $\pi[n,\ell]$ over $\ell=1,\dots,M$.

We begin by initializing every $\pi[q,\ell]$ to infinity. For $q=0$ we define $\pi[0,\ell]=0$ for every every $\ell=0,\dots,M$. Therefore, our initialization is as follows.
\[
\pi[q,\ell]\leftarrow
\begin{cases}
0 & \mbox{if $q=0$;} \\
\infty & \mbox{otherwise.}
\end{cases}
\]


Now, suppose that $q>0$ and we have computed all $\pi[i,j]$ for $i=0,\dots,q-1$. 
For any given $\ell$, we compute $\pi[q,\ell]$ as follows. We consider three cases. 

\caseparagraph{Case 1}{$\ell=0$.}
In this case, the only set $P$ is the empty set, and its cost is given by 
\[
\pi[q,0]\leftarrow\sum_{i=1}^q|\cells(A=\alpha_i)|\,.
\]

\caseparagraph{Case 2}{$\ell>0$ and $\cells(B=\alpha_i)$ is empty.} In this case, we take the minimum of two options: 
\begin{enumerate}
    \item $\alpha_q$ is a $B$-point; then the optimal $P$ includes $\alpha_k$ (for a unit cost), plus $\ell-1$ other $B$-points that optimally cover $\alpha_1,\dots,\alpha_{q-1}$. The cost is 
    $\pi[q-1,\ell-1]$ plus one unit.
    \item $\alpha_q$ is not a $B$-point; hence, the optimal $P$ of size $\ell$ is the optimal such $P$ for $\alpha_1,\dots,\alpha_{q-1}$, and the cost is the cost of $P$, namely $\pi[q-1,\ell]$, plus the size $|\cells(A=\alpha_q)|$.   
\end{enumerate}
Hence, in this case we define:
\[
\pi[q,\ell]\leftarrow \min\set{\pi[q-1,\ell-1]+1\,,\,\pi[q-1,\ell]+|\cells(A=\alpha_q)|}
\]

\caseparagraph{Case 3}{$\ell>0$ and $\cells(B=\alpha_i)$ is nonempty.} In this case, we again take the minimum of two options: 
\begin{enumerate}
    \item $\alpha_q$ is a $B$-point; then the situation is similar to the first option of the previous case, except that we need not pay the unit for $\alpha_q$ being a $B$-point (as it is not counted in the right addend of \cref{eq:costP}). The cost is then
    $\pi[q-1,\ell-1]$.
    \item $\alpha_k$ is not a $B$-point; hence, the cost is the same as the second option of the previous case. 
\end{enumerate}
Hence, in this case, we define:
\[
\pi[q,\ell]\leftarrow\min\set{\pi[q-1,\ell-1]\,,\,\pi[q-1,\ell]+|\cells(A=\alpha_q)|}
\]
The proof of correctness is by showing that whenever we consider $q$, the above assignments to $\pi[q,\ell]$ are correct, that is, $\pi[q,\ell]$ is indeed the minimum cost of a any set $P\subseteq\set{\alpha_1,\dots,\alpha_q}$ of $\ell$ $B$-points, 
according to \cref{eq:costP},
where the sum goes from $i=1$ to $i=q$.
This is done by induction that straightforwardly follows the explanations of the dynamic programming.

}


==> extensions.tex <==
\section{Extensions}
\subsection{The Maximum Norm}
Next, we prove a similar result for $\costmax$.

\begin{theorem}
    Let $(\signature,\Gamma)$ be a schema. Given an inconsistent metric database $(M,d,D)$, an optimal repair of $(M,d,D)$ on $\costmax$ can be computed in polynomial time for the line domain.
\end{theorem}
\begin{proof}
    As in the case of $\costsum$, we compute an optimal $E$ repair of $(M,d,D)$ on $\costmax$ using dynamic programming. The procedure is very similar to the one for $\costsum$, with one main difference: instead of using summation in the formulas, here we use $\max$.
As in the case of $\costsum$, we denote by $V^{D'}_r$, the cost $\costmax(D',E',d)$ of an optimal repair $E'$ of the prefix $D'$ in $\{v_1,\dots,v_r\}$, where the set $\{v_1,\dots,v_r\}$ determines the values that we are allowed to use in the repair. Our goal is to compute the value $V^{D}_n$.
We show how to compute the value $V^{D'}_r$ using dynamic programming. We have the following:
     \begin{enumerate}
            \item If $D'=\emptyset$, then $V^{D'}_r=0$. 
            \item  If $D'\neq\emptyset$ and $r<1$, then $V^{D'}_r=\infty$.
            \item Otherwise,            $$V^{D'}_r=\min_{\substack{D''\in \mathcal{P}(D')\\\cells(D'\setminus D'')\models\Gamma}}\left[ \max\left(V^{D''}_{r-1},\max_{c\in\cells(D'\setminus D'') }d(D'(c),v_r)\right)\right].\,$$
       \end{enumerate}
       The correctness again relies on the two observation mentioned in the proof for $\costsum$, and the complexity analysis is the same; hence, we do not elaborate on them here.
\end{proof}

\subsection{Bi-Objective Optimization}
We may also look at the bi-objective variant of our optimization problem, where we are interested in two intervention costs. For that, we adopt the so-called \e{$\epsilon$-constrained method} and define it as follows. Let $(\sigr,\Gamma)$ be a schema, and 
let $\kappa$ and $\kappa'$ be two intervention costs. Let $D$ be an inconsistent database, and $\tau'\geq 0$ be a number (playing the role of $\epsilon$). 
A repair is optimal on $\kappa$ under $\kappa'\leq\tau'$ if $E$ is a
$(\kappa'\leq\tau')$-repair with a minimal $\kappa(D,E)$. 

As an example, a repair is optimal on $\costsum$ under $(\costmax\leq\epsilon)$ if it is a repair with minimal total shift, assuming we allow updates of up to $\epsilon$. As another example, a repair is optimal on $\costmax$ under $(\costnum\leq k)$ if it is a repair with minimal tolerance, assuming that at most $k$ updates are allowed.

We then get the following corresponding problems, where we fix the schema $(\sigr,\Gamma)$ and the intervention costs $\kappa$ and $\kappa'$:
\begin{itemize}
    \item \textbf{Optimization problem:} given an inconsistent database $D$ and $\tau'>0$, find a repair $E$ that is optimal on $\kappa$ under $(\kappa'\leq\tau')$.
    \item \textbf{Decision problem:} given an inconsistent database $D$ and thresholds $\tau,\tau'\geq 0$, determine wheteher there exists a repair $E$ that is both a $(\kappa\leq\tau)$-repair and a 
    $(\kappa'\leq\tau')$-repair.
\end{itemize}

\subsection{Beyond a Single UID}

The following proposition states that any algorithm for a single UID applies immediately to a (common) more general case.

\begin{proposition}
Let $(\sigr,\Gamma)$ be a schema. Suppose that every UID $R.A\subseteq S.B$ in $\Gamma$ is such that no other UID in $\Gamma$ uses $R.A$ (not on the left side and not on the right side). Let $\kappa$ and $\kappa'$ be intervention costs among $\costnum$, $\costsum$ and $\costmax$, and let $\alpha\geq 1$ be a number.
\begin{itemize}
    \item If we can find in polynomial time a repair that is $\alpha$-optimal on $\kappa$ for any schema with a single UID, then we can do so for $(\sigr,\Gamma)$.
    \item Similarly, if we can find in polynomial time a repair that is $\alpha$-optimal on $\kappa$ under $(\kappa'\leq\tau')$ (where $\tau'$ is given)  
    for any schema with a single UID, then we can do so for $(\sigr,\Gamma)$.
\end{itemize}
\end{proposition}
\begin{proof}
 TBD   
\end{proof}




==> line_backup.tex <==
In this section, we consider the one-dimensional space $(M,d)$, wherein all points reside along a single straight line. For every two points $x,y\in M$, we have that
$d(x,y)=|x-y|$.
We start with the simplest case, where $\Gamma$ consists of a single UID, and show that in this case, for $\costsum$, quality is not compromised when repairs are required to be non-inventive.
\begin{proposition}\label{prop:sum_line_non_inventive}
    Let $(\sigr,\Gamma)$ be a schema such that $\Gamma$ consists of a single UID, $D$ an inconsistent database, and $\tau\geq 0$ a number. If there is a $(\costsum\leq\tau)$-repair, then there is also a $(\costsum\leq\tau)$-repair that is non-inventive.
\end{proposition}
\begin{proof}
    Assume that the single UID of $\Gamma$ is $R.A\subseteq S.B$. Let $E$ be a $(\costsum\leq\tau)$-repair that is inventive. We show how we can transform it into a $(\costsum\leq\tau)$-repair $E'$ that is non-inventive. Note that $E$ is an inventive repair if and only if there is at least one cell $(i,B)$ such that $E[i,B]\not\in\vals(D)$; this holds since $E$ is consistent, and so for every cell $(j,A)$ such that $E[j,A]\not\in\vals(D)$, there must be a cell $(i,B)$ with $E[j,A]=E[i,B]$.
    Let $(i,B)$ be a cell such that $E[i,B]\not\in\vals(D)$, and let $(j_1,A),\dots,(j_n,A)$ be all the cells over the attribute $A$ such that $E[j_1,A]=\dots=E[j_n,A]=E[i,B]$. Clearly, if no such cells exist, then we can restore the original value of the cell $(i,B)$ from $D$ without violating $\Gamma$ and while decreasing the cost. Hence, from now on, we assume that $n\ge 1$.

    Since $E[i,B]\not\in\vals(D)$, it must be the case that $E[j_k,A]\neq D[j_k,A]$ for every $k\in\{1,\dots,n\}$. We assume, without loss of generality, that the values $D[j_1,A],\dots,D[j_n,A]$ are arranged sequentially along the line, from left to right. If $E[i,B]$ is located to the right of $D[j_n,A]$, then by defining $E'[i,B]=D[j_n,A]$, we obtain \[d(D[j_k,A],E'[i,B])= d(D[j_k,A],E[i,B])-d\] for any $k\in\{1,\dots,n\}$, where $d=d(E'[i,B],E[i,B])$. For the cell $(i,B)$, we either have that \[d(D[i,B],E'[i,B])= d(D[i,B],E[i,B])-d,\text{ or}\] \[d(D[i,B],E'[i,B])= d(D[i,B],E[i,B])+d;\] however, since $n\ge 1$, defining $E'[j_k,A]=E'[i,B]$ for all $k\in\{1,\dots,n\}$ does not increase the total cost compared to $E$. Similarly, If $E[i,B]$ is located to the left of $D[j_1,A]$, we  define $E'[i,B]=D[j_1,A]$ and $E'[j_k,A]=E'[i,B]$ for all $k\in\{1,\dots,n\}$.

    Finally, if $E[i,B]$ is located between $D[j_p,A]$ and $D[j_{p+1},A]$ for some $p\in\{1,\dots,n-1\}$, then we consider four cases:
    \begin{enumerate}
        \item if $p>n-p$, we define $E'[i,B]=D[j_p,A]$,
        \item if $p<n-p$, we define $E'[i,B]=D[j_{p+1},A]$,
        \item if $p=n-p$ and $D[i,B]$ is located to the left of $D[j_{p},A]$, we define $E'[i,B]=D[j_p,A]$,
         \item if $p=n-p$ and $D[i,B]$ is located to the right of $D[j_{p+1},A]$, we define $E'[i,B]=D[j_{p+1},A]$,
         \item if $p=n-p$ and $D[i,B]$ is located between $D[j_p,A]$ and  $D[j_{p+1},A]$, we define $E'[i,B]=D[i,B]$.
    \end{enumerate}
    We have that:
    \[d(D[j_k,A], E'[i,B])=d(D[j_k,A], E[i,B])-d\text{ or}\]
    where $d=d(E[i,B],E'[i,B])$, for all $k\in\{1,\dots,p\}$ if we define $E'[i,B]=D[j_p,B]$, or for all $k\in\{p+1,\dots,n\}$ if we define $E'[i,B]=D[j_{p+1},B]$, and
    \[d(D[j_k,A], E'[i,B])=d(D[j_k,A], E[i,B])+d\]
    for all $k\in\{1,\dots,n\}$, for all $k\in\{p+1,\dots,n\}$ if we define $E'[i,B]=D[j_p,B]$, or for all $k\in\{1,\dots,p\}$ if we define $E'[i,B]=D[j_{p+1},B]$. In the first four cases, we also have that:
    \[d(D[i,B], E'[i,B])=d(D[i,B], E[i,B])-d\text{ or}\]
    \[d(D[i,B], E'[i,B])=d(D[i,B], E[i,B])+d.\]
   and one can easily verify that the number of cells for which the value decreases by $d$ in $E'$ compared to $E$ is higher or equal to the number of cells for which the value increases by $D$; hence, these modifcations do not increase the cost. In the fifth case, we have that $d(D[i,B], E'[i,B])=0$, and since $p=n-p$, the number of cells $(j_k,A)$ for which 
    \[d(D[j_k,A], E'[i,B])=d(D[j_k,A], E[i,B])-d\]
 equals the number of cells for which \[d(D[j_k,A], E'[i,B])=d(D[j_k,A], E[i,B])+d;\]
 thus, we do not increase the cost.
   We can apply this process to each cell $(i,B)$ with $E[i,B]\not\in\vals(D)$, one by one, and obtain a non-inventive repair $E'$ with $\costsum(D,E')\le\costsum(D,E)$; hence, $E'$ is a $(\costsum\leq\tau)$-repair and that concludes our proof.
\end{proof}

Using Proposition~\ref{prop:sum_line_non_inventive} we now prove that an optimal repair of $D$ on $\costsum$ can be computed in polynomial time.

\begin{theorem}
    Let $(\sigr,\Gamma)$ be a schema such that $\Gamma$ consists of a single UID. Given an inconsistent database $D$, an optimal repair of $D$ on $\costsum$ can be computed in polynomial time.
\end{theorem}
\begin{proof}
    We start with $\costsum$, and compute an optimal $E$ repair of $D$ on $\costsum$ using dynamic programming. Assume that the single UID of $\Gamma$ is $R.A\subseteq S.B$. We assume that the ids of $\rids(D)$ that are mapped to an $R$-record are $j_1,\dots,j_m$ and that the ids that are mapped to an $S$-record are $i_1,\dots,i_p$. We also assume that $\vals(D)=\{v_1,\dots,v_n\}$.
    Proposition~\ref{prop:sum_line_non_inventive} implies that we can assume $E[j_k,A]\in\vals(D)$ for every $k\in\{1,\dots,m\}$ and $E[i_k,B]\in\vals(D)$ for every $k\in\{1,\dots,p\}$.
    We also assume, without loss of generality, that the values $v_1,\dots,v_n$ are arranged sequentially along the line, from left to right, and the same holds for the values $D[j_1,A],\dots,D[j_m,A]$ and $D[i_1,B],\dots,D[i_p,B]$. 
     
    We now describe the process for computing the cost of an optimal repair. By recording all the decisions made throughout the procedure (i.e.,~mappings of cells to values), we can derive the repair itself.
    We denote by $P_{k,r}$ the cost $\costsum(D',E')$ of a repair $E'$ of $D'$, where:
    \begin{enumerate}
        \item $E'[i_k,B]=v_r$,
        \item $\rids(D')$ contains only the ids $j_t$ (among those that are mapped to an $R$-record) for which $D[j_t,A]$ is located to the left of (or on) $v_r$, only the ids $i_1,\dots,i_k$ (among those that are mapped to an $S$-record, and all the ids that are mapped to $T$-records for $T\in(\sigr\setminus\{R,S\})$,
        \item $\costsum(D',E')$ is minimal across all repairs of $D'$ that satisfy property (1). 
    \end{enumerate}
    An easy observation is that in such a repair $E'$ it cannot be the case that $E'[i_k,B]=v_r$ while $E'[i_\ell,B]=v_t$ for some $\ell<k$ and $t>r$; otherwise, we can swap the values (i.e.~change the value of the cell $(i_k,B)$ to $v_t$ and the value of the cell $(i_\ell,B)$ to $v_r$) without increasing the cost. This holds since  $D[i_k,B]$ is located to the right of $D[i_\ell,B]$, while $v_r$ is located to the left of $v_t$. Hence, we can always assume that in $E'$, the right-most value of some cell corresponding to the attribute $B$ is $v_r$. It is now not hard to see that our goal is to compute the following value:
    \[\min_{1\le r\le n} \left(P_{p,r}+\sum_{[j_t,A]\in S_{>r}}d(D[j_t,A],v_r)\right)\]
    where $S_{>r}=\{(j_t,A)\mid D[j_t,A]\text{ is located to the right of }v_r\}$.

    We now show how to compute the value $P_{k,r}$.
    \[
        P_{k,r}=
        \begin{cases}
          \sum_{[j_t,A]\in S_{\le r}}d[D[j_t,A],v_r] & k=1;\\
          \min_{\ell\le r}\left(P_{k-1,\ell}+\sum_{[j_t,A]\in S_{[\ell,r]}}\min(d(D[j_t,A],v_\ell),d(D[j_t,A],v_r))\right) & k>1;\\
        \end{cases}
    \]
    where $S_{\le r}=\{(j_t,A)\mid D[j_t,A]\text{ is located to the left of (or on) }v_r\}$, and $S_{[\ell,r]}=\{(j_t,A)\mid D[j_t,A]\text{ is located between }v_\ell\text{ and }v_r\}$. The first case refers to the situation where we only consider one cell corresponding to the attribute $B$ and set its value to $v_r$; in this case, all the cells corresponding to the attribute $A$ that we consider must contain the same value. In the second case, we go over all possible values $v_\ell$ for the cell $(i_{k-1},B)$ (as aforementioned, if we define $E'[i_k,B]=v_r$, we will not define $E'[i_{k-1},B]=v_\ell$ for some $\ell>r$), and add to the value $P_{k-1,\ell}$ the cost of changing the values of the cells $(j_t,A)$ such that $D[j_t,A]$ is located between $v_\ell$ and $v_r$ to either $v_\ell$ or $v_r$; we choose the options with the lower cost for each cell. 
    Clearly, there is no need to consider changing the value of the cells $(j_t,A)$ such that $D[j_t,A]$ is located to the left of (or on) $v_\ell$ to $v_r$, as this can only increase the cost of the repair.

    This completes the description of the algorithm. The correctness is a straightforward conclusion
    from this description. Clearly, we can compute each value $P_{1,r}$ in polynomial time, and there are lineraly many such values. Similarly, for $k>1$, assuming that we have already computed the values $P_{k-1,r}$, it is rather straightforward that we can compute the value $P_{k,r}$ in polynomial time. Since the total number of values that we have to compute is $p\times n$ (i.e.,~a polynomial), and each one of the requires polynomial time, we conclude that the algorithm runs in polynomial time.
\end{proof}

Next, we consider $\costmax$, and show that for this cost function, it might be the case that every optimal repair is inventive; however, we only need to invent polynomially many values.

\begin{lemma}\label{lem:max_line_linear_inventive}
    Let $(\sigr,\Gamma)$ be a schema such that $\Gamma$ consists of a single UID, $D$ an inconsistent database, and $\tau\geq 0$ a number. If there is a $(\costmax\leq\tau)$-repair, then there is also a $(\costmax\leq\tau)$-repair $E$ such that for every attribute $A$ and cell $(i,A)$ of $D$ one of the following holds:
    \begin{itemize}
        \item $E[i,A]\in\vals(D)$, or
        \item $E[i,A]$ is located midway between two values of $\vals(D)$.
    \end{itemize}
\end{lemma}
\begin{proof}
 Assume that the single UID of $\Gamma$ is $R.A\subseteq S.B$. Let $E$ be a $(\costsum\leq\tau)$-repair. We show how we can transform it into a $(\costsum\leq\tau)$-repair $E'$ that satisfies the required property. 
    Let $(i,B)$ be a cell such that $E[i,B]\not\in\vals(D)$, and let $(j_1,A),\dots,(j_n,A)$ be all the cells over the attribute $A$ such that $E[j_1,A]=\dots=E[j_n,A]=E[i,B]$. Clearly, if no such cells exist, then we can restore the original value of the cell $(i,B)$ from $D$ without violating $\Gamma$ and while decreasing the cost. Hence, from now on, we assume that $n\ge 1$.

    Since $E[i,B]\not\in\vals(D)$, it must be the case that $E[j_k,A]\neq D[j_k,A]$ for every $k\in\{1,\dots,n\}$. We assume, without loss of generality, that the values $D[j_1,A],\dots,D[j_n,A]$ are arranged sequentially along the line, from left to right. If $D[i,B]$ is located to the right of $D[j_n,A]$, then by defining the value  $E'[i,B]$ as the midpoint between $D[i,B]$ and $D[j_1,A]$ (and defining $E'[j_k,A]=E'[i,B]$ for all $k\in\{1,\dots,n\}$) we can only decrease the cost compared to $E$. This holds since the longest distance in this case (among the distances $d(D[j_k,A],E'[i,B])$ for $k\in\{1,\dots,n\}$ and $d(D[i,B],E'[i,B])$) is between $D[j_1,A]$ and $E'[i,B]$; if $E'[i,B]$ is the midpoint between these two values, then the distance is $\frac{1}{2}\times d(D[j_1,A],D[i,B])$, if we move it to the left, this increases the distance between $D[i,B]$ and $E'[i,B]$, and if we move it to the right, the distance between $D[j_1,A]$ and $E'[i,B]$ increases. Since with $\costmax$ we consider only the maximal distance between two values, the best option is the midpoint. Similarly, in the case where $D[i,B]$ is located to the left of $D[j_1,A]$, we define the value $E'[i,B]$ as the midpoint between $D[i,B]$ and $D[j_n,A]$. 

    Finally, if $D[i,B]$ is located between $D[j_1,A]$ and $D[j_n,A]$, then we define the value $E'[i,B]$ as the midpoint between $D[j_1,A]$ and $D[j_n,A]$. In this case, the longest distance is between $D[j_1,A]$ (and  $D[j_n,A]$) and $E'[i,B]$; if $E'[i,B]$ is the midpoint between these two values, then the distance is $\frac{1}{2}\times d(D[j_1,A],D[j_n,A])$, if we move it to the left, this increases the distance between $D[j_n,A]$ and $E'[i,B]$, and if we move it to the right, the distance between $D[j_1,A]$ and $E'[i,B]$ increases. Hence, the best option is the midpoint. We can apply this process to each cell $(i,B)$ with $E[i,B]\not\in\vals(D)$, one by one, and obtain a repair $E'$ that is a $(\costsum\leq\tau)$-repair and satisfies the required property, and that concludes our proof.
\end{proof}

We now use~\cref{lem:max_line_linear_inventive} to show the following.

\begin{theorem}
    Let $(\sigr,\Gamma)$ be a schema such that $\Gamma$ consists of a single UID. Given an inconsistent database $D$, an optimal repair of $D$ on $\costmax$ can be computed in polynomial time.
\end{theorem}
\begin{proof}
    As in the case of $\costsum$, we compute an optimal $E$ repair of $D$ on $\costmax$ using dynamic programming. Assume that the single UID of $\Gamma$ is $R.A\subseteq S.B$. We assume that the ids of $\rids(D)$ that are mapped to an $R$-record are $j_1,\dots,j_m$ and that the ids that are mapped to an $S$-record are $i_1,\dots,i_p$. We also assume that $V=\{v_1,\dots,v_n\}$ is the set of all values that are in $\vals(D)$ or located midway between two values of $\vals(D)$ (note that there $\vals(D)+\frac{\vals(D)\times(\vals(D)-1)}{2}$ such values).
\cref{lem:max_line_linear_inventive} implies that we can assume $E[j_k,A]\in V$ for every $k\in\{1,\dots,m\}$ and $E[i_k,B]\in V$ for every $k\in\{1,\dots,p\}$.
    We also assume, without loss of generality, that the values $v_1,\dots,v_n$ are arranged sequentially along the line, from left to right, and the same holds for the values $D[j_1,A],\dots,D[j_m,A]$ and $D[i_1,B],\dots,D[i_p,B]$. 
     
    We now describe the process for computing the cost of an optimal repair (which is very similar to the one for $\costsum$). By recording all the decisions made throughout the procedure (i.e.,~mappings of cells to values), we can derive the repair itself.
    We denote by $P_{k,r}$ the cost $\costmax(D',E')$ of a repair $E'$ of $D'$, where:
    \begin{enumerate}
        \item $E'[i_k,B]=v_r$,
        \item $\rids(D')$ contains only the ids $j_t$ (among those that are mapped to an $R$-record) for which $D[j_t,A]$ is located to the left of (or on) $v_r$, only the ids $i_1,\dots,i_k$ (among those that are mapped to an $S$-record, and all the ids that are mapped to $T$-records for $T\in(\sigr\setminus\{R,S\})$,
        \item $\costmax(D',E')$ is minimal across all repairs of $D'$ that satisfy property (1). 
    \end{enumerate}
    An easy observation is that in such a repair $E'$ it cannot be the case that $E'[i_k,B]=v_r$ while $E'[i_\ell,B]=v_t$ for some $\ell<k$ and $t>r$; otherwise, we can swap the values (i.e.~change the value of the cell $(i_k,B)$ to $v_t$ and the value of the cell $(i_\ell,B)$ to $v_r$) without increasing the cost. This holds since  $D[i_k,B]$ is located to the right of $D[i_\ell,B]$, while $v_r$ is located to the left of $v_t$. Hence, we can always assume that in $E'$, the right-most value of some cell corresponding to the attribute $B$ is $v_r$. It is now not hard to see that our goal is to compute the following value:
    \[\min_{1\le r\le n} \left(P_{p,r}+\max_{[j_t,A]\in S_{>r}}d(D[j_t,A],v_r)\right)\]
    where $S_{>r}=\{(j_t,A)\mid D[j_t,A]\text{ is located to the right of }v_r\}$.

    We now show how to compute the value $P_{k,r}$.
    \[
        P_{k,r}=
        \begin{cases}
          \max_{[j_t,A]\in S_{\le r}}d[D[j_t,A],v_r] & k=1;\\
          \min_{\ell\le r}\left(P_{k-1,\ell}+\max_{[j_t,A]\in S_{[\ell,r]}}\min(d(D[j_t,A],v_\ell),d(D[j_t,A],v_r))\right) & k>1;\\
        \end{cases}
    \]
    where $S_{\le r}=\{(j_t,A)\mid D[j_t,A]\text{ is located to the left of (or on) }v_r\}$, and $S_{[\ell,r]}=\{(j_t,A)\mid D[j_t,A]\text{ is located between }v_\ell\text{ and }v_r\}$. The The only difference compared to $\costsum$ is that we use $\max$ instead of $\sum$ in the computation; the correctness and complexity analysis are very similar, and we do not discuss them again here.
\end{proof}

==> old-infinite.tex <==
Our proofs will use the following proposition, which bounds the loss in quality when restricted to use only original data points.
\begin{proposition}\label{prop:non-inventive}
Let $\Gamma$ be a set of UIDs, $D$ an inconsistent database, and $\tau\geq 0$ a number.
\begin{enumerate}
    \item Suppose that $\kappa$ is $\costnum$. If there is a $(\kappa\leq\tau)$-repair, then there is also a $(\kappa\leq\tau)$-repair that is non-inventive.
     \item Suppose that $\kappa$ is $\costmax$ or $\costsum$. If there is a $(\kappa\leq\tau)$-repair, then there is also a $(\kappa\leq2\tau)$-repair that is non-inventive.
\end{enumerate}
\end{proposition}
\begin{proof}
Part~1 is straightforward: given any repair $E$, we choose an arbitrary value $v$ in $\vals(D)$, and update every cell of $E$ with a value outside of $\vals(D)$ to be the chosen value $v$. Note that $E$ continues to be consistent. Moreover, the cost $\costnum(D,E)$ does not increase due to this replacement, since every cell with a changed value is also changed before the replacement.

For Part~2, suppose that $\kappa$ is either $\costmax$ or $\costsum$. Let $E$ be a repair. We will construct a non-inventive repair $E'$ such that
$\kappa(D,E')\leq2\cdot\kappa(D,E)$. To construct $E'$, we update every cell with a value $a$ outside of $\vals(D)$.
For that, we apply the following change to $E$, for every $a\in\vals(E)\setminus\vals(D)$, until no such $a$ exists. 
Let $c_m\in E^{-1}(a)$ be a cell such that $\Delta(D(c_m),a)$ is minimal among the cells $c\in E^{-1}(a)$. Hence, $c_m$ is the cell that has the least cost of update among those of $E^{-1}(a)$. We replace in $E$ the value of every cell in $E^{-1}(a)$ with the value $D(c_m)$. 

Again, it is clearly the case that $E'$ is consistent since $E'$ satisfies all pairwise equalities that $E$ satisfies. Also,
 note that for every $c\in E^{-1}(a)$ it holds that
$$\Delta(D(c),E'(c))
\leq \Delta(D(c),E(c))+ \Delta(E(c),E'(c))
\leq 2\cdot \Delta(D(c),E(c))\,.
$$
The first inequality is due to the triangle inequality. The second inequality is due to the construction above where  $\Delta(E(c),E'(c))$ is the same as $\Delta(a,D(c_m))$, and $\Delta(a,D(c_m))=\Delta(D(c_m),a)$ is at most $\Delta(D(c),a)=\Delta(D(c),E(c))$ due to symmetry.  We conclude that 
$\Delta(D(c),E'(c))$ is at most $2\cdot \Delta(D(c),E(c))$ and then Part~2 of the proposition immediately follows for both $\costmax$ and $\costsum$.
\end{proof}

We show that for the line domain, in the case of $\costsum$, quality is not compromised when repairs are required to be non-inventive.

\begin{proposition}\label{prop:sum_line_non_inventive}
    Let $\Gamma$ be a set of UIDs, $D$ an inconsistent database, and $\tau\geq 0$ a number. For the line domain, if there is a $(\costsum\leq\tau)$-repair, then there is also a $(\costsum\leq\tau)$-repair that is non-inventive.
\end{proposition}
\begin{proof}
    $(\costsum\leq\tau)$-repair of $D$. Let $c$ be a cell such that $E(c)\not\in\vals(D)$. Let $c_1,\dots,c_n$ be all the cells such that $E(c_\ell)=E(c)$ (including the cell $c$ itself). We assume, without loss of generality, that the original values of these cells are arranged sequentially along the line, from left to right; that is, for every $\ell\in\{1,\dots,n-1\}$, it holds that $D(c_\ell)$ is located to the left of $D(c_{\ell+1})$ (hence, $D(c_\ell)\le D(c_{\ell+1})$).
    We show how we can transform $E$ into a $(\costsum\leq\tau)$-repair $E'$, such that $E'(c_\ell)\in\vals(D)$ for every $\ell\in\{1,\dots,n\}$. By repeatedly applying this process to each group of cells with a value outside $\vals(D)$, we can obtain a non-inventive repair $E''$ with $\costsum(D,E'')\le\costsum(D,E)$.

    If $E(c)$ is located to the right of $D(c_n)$, then by defining $E'(c_\ell)=D(c_n)$ for every $\ell\in\{1,\dots,n\}$, we clearly do not introduce any violations of the constraints, and for every $\ell\in\{1,\dots,n\}$ we have that: \[\Delta(D(c_\ell),E'(c))= \Delta(D(c_\ell),E(c))-\delta.\]  where $\delta=\Delta(E'(c),E(c))$. Hence, $\costsum(D,E')\le\costsum(D,E)$. Similarly, If $E(c)$ is located to the left of $D(c_1)$, then we can define $E'(c_\ell)=D(c_1)$ for all $\ell\in\{1,\dots,n\}$, and obtain a repair $E'$ with $\costsum(D,E')\le\costsum(D,E)$. 

    Finally, if $E(c)$ is located between $D(c_k)$ and $D(c_{k+1})$ for some $k\in\{1,\dots,n-1\}$, then we define $E'(c_\ell)=D(c_k)$ for every $\ell\in\{1,\dots,n\}$ if $k\le n-k$ or $E'(c_\ell)=D(c_{k+1})$ for every $\ell\in\{1,\dots,n\}$ if $k< n-k$. In the first case, we have that \[\Delta(D(c_\ell),E'(c))= \Delta(D(c_\ell),E(c))-\delta.\] for every $\ell\in\{1,\dots,k\}$, where $\delta=\Delta(E'(c),E(c))$, and
    \[\Delta(D(c_\ell),E'(c))= \Delta(D(c_\ell),E(c))+\delta.\] for every $\ell\in\{k+1,\dots,n\}$. Since $k\le n-k$, the number of cells for which the distance decreases is not smaller than the number of cells for which the value increases, and $\costsum(D,E')\le\costsum(D,E)$. Similarly, in the second case, we have that \[\Delta(D(c_\ell),E'(c))= \Delta(D(c_\ell),E(c))+\delta.\] for every $\ell\in\{1,\dots,k\}$, and
    \[\Delta(D(c_\ell),E'(a))= \Delta(D(c_\ell),E(c))-\delta.\] for every $\ell\in\{k+1,\dots,n\}$. Since $n-k>k$, the number of cells for which the distance decreases is larger than the number of cells for which the value increases, and $\costsum(D,E')\le\costsum(D,E)$. This concludes our proof. 
\end{proof}

Next, we consider $\costmax$, and show that for this cost function, it might be the case that every optimal repair is inventive; however, we only need to invent polynomially (specifically, $O(|\vals(D)|^2)$) many values.

\begin{lemma}\label{lem:max_line_poly_inventive}
    Let $(\sigr,\Gamma)$ be a schema, $D$ an inconsistent database, and $\tau\geq 0$ a number. If there is a $(\costmax\leq\tau)$-repair, then there is also a $(\costmax\leq\tau)$-repair $E$ such that for every attribute $A$ and $A$-cell $c$ of $\cells(D)$ one of the following holds:
    \begin{itemize}
        \item $E(c)\in\vals(D)$, or
        \item $E(c)$ is located midway between two values of $\vals(D)$.
    \end{itemize}
\end{lemma}
\begin{proof}
    Let $E$ be a $(\costmax\leq\tau)$-repair of $D$. Let $c$ be a cell of $\cells(D)$ such that $E(c)=v$ with $v\not\in\vals(D)$ and $v$ is not located midway between two values of $\vals(D)$. Let $c_1,\dots,c_n$ be all the cells such that $E(c_\ell)=v$ (including the cell $c$ itself). We assume, without loss of generality, that the original values of these cells are arranged sequentially along the line, from left to right; that is, for every $\ell\in\{1,\dots,n-1\}$, it holds that $D(c_\ell)$ is located to the left of (or on) $D(c_{\ell+1})$.
    We show how we can transform $E$ into a $(\costmax\leq\tau)$-repair $E'$, such that $E'(c_\ell)\in\vals(D)$ or $E'(c_\ell)$ is located midway between two values of $\vals(D)$, for every $\ell\in\{1,\dots,n\}$. By repeatedly applying this process to each group of cells with a value outside $\vals(D)$, we can obtain a repair $E''$ that satisfies the desired property, with $\costmax(D,E'')\le\costmax(D,E)$.

    For every $\ell\in\{1,\dots,n\}$, we define $E'(c_\ell)$ as the midpoint $v'$ between $D(c_1)$ and $D(c_n)$. By doing so we do not introduce violations of the UIDs, as all these cells are still associated with the same value. In this case, the longest distance, among the distances $d(D(c_\ell),E'(c_\ell)$ for $\ell\in\{1,\dots,n\}$, is between $D(c_1)$ and $E'(c_1)$ and $D(c_n)$ and $E'(c_n)$. It is also rather straightforward that the longest distance, among the distances $d(D(c_\ell),E(c_\ell))$ for $\ell\in\{1,\dots,n\}$, is either between $D(c_1)$ and $E(c_1)$ or between $D(c_n)$ and $E(c_n)$. If $v$ is located to the left of $v'$, then the longest distance is between $D(c_n)$ and $E(c_n)$, and we have that:
    \[d(D(c_n),E'(c_n))\le d(D(c_n),E(c_n)).\]
    If $v$ is located to the right of $v'$, then the longest distance is between $D(c_1)$ and $E(c_1)$, and we clearly have that:
    \[d(D(c_1),E'(c_1))\le d(D(c_1),E(c_1)).\]
    In both cases, it holds that:
    \[\max_{1\le \ell\le n}d(D(c_\ell),E'(c_\ell))\le \max_{1\le \ell\le n}d(D(c_\ell),E(c_\ell));\] hence, $\costmax(D,E')\le\costmax(D,E)$, and this concludes our proof.
\end{proof}



Nevertheless, we can adapt the proof of \Cref{prop:non-inventive} to important cases, such as the Euclidian space, without making any assumption on the global $\Gamma$. For that, we need to be able to produce enough points that are close to the points of $D$, and then avoid reusing points. Formally, we will say that $(M,\delta)$ has \e{efficient neighborhood generation} if we can solve the following problem in polynomial time in $1/\epsilon$ and $n$: given a point $v$, produce $n$ \e{distinct} points $u\in M$ such that $\delta(v,u)\leq\epsilon$. Clearly, this is the case for every $l_p$-metric.

\begin{proposition}\label{prop:small-inventive}
Let $(M,\delta)$ be an infinite metric space and $\Gamma$ a global coincidence constraint. Suppose that $(M,\delta)$ has efficient neighborhood generation. Given an inconsistent database $D$ and a number $\epsilon>0$, one can construct in polynomial time a set $M'\subseteq M$ such that $|M'|\leq |D|\cdot |\vals(D)|$ and, moreover, there is a $(2+\epsilon)$-optimal repair $E$ such that $\vals(E)\subseteq M'$. 
\end{proposition}
\begin{proof}
Let $\eta'$ be the minimal distance between two     
\end{proof}

==> old.tex <==
%For general metrics, we later rely on embeddings to tree metrics. (See ...) %\Cref{}.)


A \e{relation signature} has the form $R(A_1,\dots,A_k)$ where $R$ is a \e{relation name} and $A_1,\dots,A_k$ are distinct \e{attribute names}.
A \e{database signature} is a finite set $\sigr$ of relation signatures with distinct relation names. If $\sigr$ contains $R(A_1,\dots,A_k)$, then we say that $k$ is the \e{arity} of $R$ and that 
$A_1,\dots,A_k$ are the attributes of $R$.

Let $\vals$ be a domain of \e{values}. A \e{record} over the database signature $\sigr$ is an expression of the form $R(a_1,\dots,a_k)$ 
for some relation signature 
$R(A_1,\dots,A_k)$ of $\sigr$ and a sequence
$(a_1,\dots,a_k)$ of values in $\vals$.
We call $R(a_1,\dots,a_k)$ an \e{$R$-record}. If $r=R(a_1,\dots,a_k)$ is a record, then we denote each value $a_i$ by $r.A_i$.


A \e{database} $D$ over $\sigr$ is a mapping from a finite set of \e{record identifiers} (or just \e{ids} for short) to facts over $\sigr$. We denote this set of ids by $\rids(D)$. Hence, $D$ is a function that maps every id $i$ to an $R$-record for some relation name $R$ of $\sigr$. We denote this record by $D[i]$.
(Note that we allow for duplicate tuples, as we do not assume that the records of different identifiers are necessarily different.) 

A \e{cell} of a database $D$ is a pair $(i,A)$ where $i\in\rids(D)$ and $A$ is an attribute of the relation of $D[i]$. By $\cells(D)$ we denote the set of all cells of $D$. If $(i,A)\in\cells(D)$, then we denote by $D[i,A]$ the value $D[i].A$ (i.e., the value that the record $i$ of $D$ has for the attribute $A$).

For a database $D$, we denote by $\vals(D)$ the \e{active domain} of $D$, that is, the set of all values that occur in $D$. In notation,
$\vals(D)\defeq\set{D[i,A]\mid (i,A)\in\cells(D)}$.


\subparagraph*{Unary Inclusion Constraint (UID).}
For a database signature $\sigr$, a UID has the form $R.A\subseteq S.B$ for some relation names $R$ and $S$ of $\sigr$ with the attributes $A$ and $B$, respectively. A database $D$ over $\sigr$ satisfies the UID $R.A\subseteq S.B$ if for every $R$-record $r$ of $D$ there is an $S$-record $s$ of $D$ such that $r.A=s.B$. The database $D$ satisfies a set $\Gamma$ of UIDs, denoted $D\models\Gamma$, if $D$ satisfies every UID of $\Gamma$. Conversely, $D$ \e{violates} $\Gamma$ if $D$ violates at least one UID of $\Gamma$, and then we denote it by $D\not\models\Gamma$.

\subparagraph*{Schema.}
In this work, a \e{schema} is a pair $(\sigr,\Gamma)$ where $\sigr$ is a database signature and $\Gamma$ is a set of UIDs over $\sigr$. In the context of a schema $(\sigr,\Gamma)$, a \e{consistent database} is a database $D$ over $\sigr$
such that $D\models\Gamma$, and an \e{inconsistent database} is a database $D$ over $\sigr$
such that $D\not\models\Gamma$.


The \e{difference} between $D$ and $E$, denoted $\Delta(D,E)$, is the numerical vector that is obtained from $\vcells(D)$ by placing instead of every cell
$(i,A)$ the distance $d(D[i,A],E[i,A])$ between the values of the corresponding cells of $D$ and $E$.


Given a database $D$, we denote by $\vcells(D)$ the sequence of all cells of $D$ according to this order.  Note that when $E$ is a repair of $D$, it holds that 
$\cells(D)=\cells(E)$ and
$\vcells(D)=\vcells(E)$. 

We will look at various computational problems that arise naturally in our framework.

\begin{itemize}
    \item \textbf{Optimization problem:} given an inconsistent database $D$, find a repair that is optimal on $\kappa$ (or an $\alpha$-approximation thereof).
    \item  \textbf{Decision problem:} given an inconsistent database $D$ and a threshold $\tau\geq 0$, determine whether there exists a $(\kappa\leq\tau)$-repair.
\end{itemize}


==> one-dimension.tex <==
\subsection{The Line Domain}

In this section, we consider the case where
$(\vals,\Delta)$ is the one-dimensional space, wherein all points reside along a single straight line. Hence, $\vals$ is the set $\mathbb{Q}$ of rational numbers, and $\Delta(x,y)=|x-y|$. We prove that an optimal repair of $D$ on $\costsum$ can be computed in polynomial time for the line domain. 

\begin{theorem}
    Let $(\signature,\Gamma)$ be a schema. Given an inconsistent metric database $(M,d,D)$, an optimal repair of $(M,d,D)$ on $\costsum$ can be computed in polynomial time for the line domain.
\end{theorem}
\begin{proof}
    We compute an optimal repair $E$ of $(M,d,D)$ on $\costsum$ using dynamic programming. We assume, without loss of generality, that the values of $M$, which we denote by $v_1,\dots,v_n$, are arranged sequentially along the line, from left to right (hence, $v_1\le\dots\le v_n$). %\Cref{prop:sum_line_non_inventive} implies that we can assume $E(c)\in\vals(D)$ for every attribute $c\in\cells(D)$. 
    We now describe the process for computing the cost of an optimal repair. By recording all the decisions made throughout the procedure (i.e.,~mappings of cells to values), we can derive the repair itself.

   We begin with an intuition on the general idea of the algorithm. The coincidence constraint essentially imposes restrictions on the cells associated with the values $v_1,\dots,v_n$, and these restrictions can be individually verified for each value.  %For example, the coincidence constraint $\Gamma_{A\sqsubseteq B}$, that corresponds to the inclusion constraint $A\sqsubseteq B$, indicates that for every $v_r$ for $r\in\{1,\dots,n\}$ one of the following holds:
   %\begin{enumerate}
    %   \item $D$ has no $A$-cell $c$ with $E(c)=v_r$ and no $B$-cell $c'$ with $E(c')=v_r$.
     %  \item $D$ has no $A$-cell $c$ with $E(c)=v_r$, but it has a $B$-cell $c'$ with $E(c')=v_r$.
     %  \item $D$ has an $A$-cell $c$ with $E(c)=v_r$ and a $B$-cell $c'$ with $E(c')=v_r$.
   %\end{enumerate}
   %\benny{Revised up to here}   
   %Therefore, it cannot be the case that for some $r\in\{1,\dots,n\}$, there is an $A$-cell $c$ with $D(c)=v_r$, but no corresponding $B$-cell $c'$ with $D(c')=v_r$. In other words, it must be the case that $p_D(v_r)\models\Gamma$. 
   Consequently, to compute a repair $E$ of $(M,d,D)$, we must arrange the cells of $D$ on the line in such a way that for every $r\in\{1,\dots,n\}$, it holds that $p_E(v_r)\models\Gamma$.
   
    Another crucial observation is that in an optimal repair $E$ of $(M,d,D)$, there are no two $A$-cells $c,c'$ for some attribute $A$ such that $D(c)<D(c')$ while $E(c)>E(c')$; otherwise, we could swap the values (i.e.~change the value $E(c)$ to $E(c')$ and the value $E(c')$ to $E(c)$) without introducing violations of constraint and while decreasing the cost. This holds since $D(c)$ is located to the left of $D(c')$ on the line, while $E(c)$ is located to the right of $E(c')$. Consequently, when arranging the cells along the line, we only need to consider cases where the order aligns with the original ordering of the cells from $D$. 
    This observation allows us to split the problem into smaller problems. Informally, if the cells of $\cells(D)$ are $c_1,\dots,c_m$, and assuming that these cells are arranged sequentially along the line, we can solve the problem for some prefix $c_1,\dots,c_\ell$ (where $1\le \ell\le m$) 
    of the sequence of cells, and then position all the cells $c_{\ell+1},\dots,c_m$ in the suffix to the right of the cells in the prefix. 
    The combination of these two observations leads to a dynamic programming procedure for computing an optimal repair, that we now formally describe.
    
Let $C\subseteq\cells(D)$. We say that $C$ is consistent (denoted $C\models\Gamma$) if $D'\models\Gamma$, where $D'$ is such that $\cells(D')=C$ and there is $v\in M$ such that $D'(c)=v$ for all $c\in\cells(D')$.
Next, assume $\signature=(A_1,\dots,A_k)$. 
For every attribute $A_j$ of $\signature$, we assume that the cells of $\cells(D[A_j])$ are $c^{j}_1,\dots,c^j_{m_j}$, and assume, without loss of generality, that these cells are arranged sequentially along the line, from left to right.
%Let $C\subseteq C_\signature$ be a set of cells that contains, for every attribute $A_j\in \signature$, the cells $(1,A_j),\dots,(\ell_{j},A_j)$ for some $0\le \ell_j\le m_j$ (if $\ell_j=0$, then $C$ contains no cells over the attribute $A_j$). 
We say that a database $D'$ is a \emph{prefix} of $D$ if for every attribute $A_j$ of $\signature$: \emph{(1)} $D'[A_j]=\{c^j_1,\dots,c^j_{\ell_j}\}$ for some $0\le \ell_j\le m_j$ (if $\ell_j=0$ then $D'[A_j]=\emptyset$) and \emph{(2)} $D'(c^j_r)=D(c^j_r)$ for all $r\in\{1,\dots,\ell_j\}$. %We define an order $D_1,\dots,D_N$ over all the prefixes of $D$, such that $i< j$ whenever $D_i$ is a prefix of $D_j$. 
Let $D_1$ and $D_2$ be two prefixes of $D$. If for every attribute $A_j$ of $\signature$, it holds that $\cells(D_2[A_j])\subseteq \cells(D_1[A_j])$, then we refer to $D_2$ as a prefix of $D_1$. The suffix of $D_2$ w.r.t.~$D_1$ is the database $D_3$ such that for every attribute $A_j$ of $\signature$, $\cells(D_3[A_j])=\cells(D_1[A_j])\setminus \cells(D_2[A_j]$), and $D_3(c)=D_1(c)$ for all $c\in \cells(D_3[A_j])$.
We denote the suffix of $D_2$ w.r.t.~$D_1$ by $D_1\setminus D_2$. For every prefix $D'$ of $D$, we denote by $\mathcal{P}(D')$ the set of all prefixes of $D'$. Note that we can construct $\mathcal{P}(D')$ in polynomial time, since the number $k$ of attributes in $\signature$ is constant in data complexity; hence, there are at most $|D|^k$ options for the values $\ell_1,\dots,\ell_k$.


%For $0\le i_1\le m_1,\dots,0\le i_k\le m_k$, the \emph{prefix} $P^{i_1,\dots,i_k}$ of $C_\signature$ consists of (possibly empty) prefixes of cell sequences from $C_\signature$, for all attributes of $\signature$; for every attribute $A_j\in \signature$, the set $P^{i_1,\dots,i_k}$ contains the cells $(1,A_j),\dots,(i_j,A_j)$ (if $i_j=0$, then it contains no cells over the attribute $A_j$).
%Let $P^{i_1,\dots,i_k}$ and $P^{\ell_1,\dots,\ell_k}$ be two prefixes of $C_\signature$. If $\ell_j\le i_j$ for every $j\in\{1,\dots,k\}$, we refer to $P^{\ell_1,\dots,\ell_k}$ as a prefix of $P^{i_1,\dots,i_k}$. We can construct the set of all prefixes of $P^{i_1,\dots,i_k}$ in polynomial time, since the number $k$ of attributes in $\signature$ is constant in data complexity; hence, there are at most $|D|^k$ options for the values $\ell_1,\dots,\ell_k$. The \emph{suffix} $S^{i_1\mid l_1,\dots,i_k\mid \ell_k}$ of $P^{i_1,\dots,i_k}$ w.r.t.~$P^{\ell_1,\dots,\ell_k}$ contains the (possibly empty) suffixes of cell sequences from $P^{i_1,\dots,i_k}$ for all attributes $A_j\in\signature$. For every attribute $A_j\in \signature$, the set $S^{i_1\mid l_1,\dots,i_k\mid \ell_k}$ contains the cells $(\ell_j+1,A_j),\dots,(i_j,A_j)$; if $i_j=\ell_j$, then it contains no cells over $A_j$. 
   
   %We denote by $S_{\signature}^{i_1,\dots,i_k}$ the set of all cells $(\ell,A_j)\in S_{\signature}$ such that $j\in\set{1,\dots,k}$ and    
   %$\ell\le i_j$. 
%    Let $C\subseteq C_{\signature}$. We say that $C$ is consistent w.r.t.~$\Gamma$ (denoted $C\models\Gamma$) if for every UID $R.A\subseteq S.B$ in $\Gamma$ and every cell $(i,A)\in C$, there exists a cell $(j,B)\in C$. 


%For a set $C\subseteq C_\signature$ and a database $E'$, we say that $C$ is consistent in $E'$ w.r.t.~$\Gamma$ (denoted $C(E')\models\Gamma$) if for every UID $R.A\subseteq S.B$ in $\Gamma$ and every cell $(i,A)\in C$, there exists a cell $(j,B)\in C$ such that $E'[i,A]=E'[j,B]$.
%if: \emph{(1)} $\rids(D)=\rids(E')$, \emph{(2)}
%for every $i\in\rids(D)$, the records $D[i]$ and $E'[i]$ have the same relation name, and \emph{(3)} $C(E')\models\Gamma$. A $C$-repair $E'$ of $D$ is optimal in $\{v_1,\dots,v_r\}$ if $E'[\ell,A_j]\in\{v_1,\dots,v_r\}$ for every cell $(\ell, A_j)\in C$ and $\costsum(D,E')$ is minimal among all $C$-repairs of $D$ satisfying this property. 
   Finally, for a prefix $D'$ of $D$ and $1\le r\le n$, 
   we say that a repair $E'$ of $(M,d,D')$ is an optimal repair of $(M,d,D')$ in $\{v_1,\dots,v_r\}$ if $E'(c)\in\{v_1,\dots,v_r\}$ for every $c\in\cells(D')$, and $\costsum(D',E',d)$ is minimal among all repairs of $(M,d,D')$ satisfying this property. 
   We denote by $V^{D'}_r$ the cost $\costsum(D',E',d)$ of an optimal repair $E'$ of $(M,d,D')$ in $\{v_1,\dots,v_r\}$.
It is now not hard to see that our goal is to compute the value $V^D_n$.
 We show how to compute the value $V^{D'}_r$ using dynamic programming. We have the following:
     \begin{enumerate}
            \item If $\cells(D')=\emptyset$, then $V^{D'}_r=0$. 
            \item  If $\cells(D')\neq\emptyset$ and $r<1$, then $V^{D'}_r=\infty$.
            \item Otherwise,            $$V^{D'}_r=\min_{\substack{D''\in \mathcal{P}(D')\\\cells(D'\setminus D'')\models\Gamma}}\left( V^{D''}_{r-1}+\sum_{c\in\cells(D'\setminus D'') }d(D'(c),v_r)\right).\,$$
            %where $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature$ is the set of cells $(\ell,A_j)\in S_\signature$ such that $i_j'+1\le \ell\le i_j$ (if $i_j'+1>i_j$, we assume that $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature$ contains no cells over $A_j$), and by $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature\models\Gamma$ we mean that by changing the values of all the cells of $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature$ to the same value we obtain an $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature$-repair of $D$.
       \end{enumerate}
   The first case refers to the situation where we consider no cells; hence, the cost is zero. The second case refers to the situation where we no longer have available positions for the remaining cells, and the cost is infinite. In the third case, we go over all possible prefixes $D''$ of $D'$ such that the suffix of $D''$ w.r.t.~$D'$ is consistent w.r.t.~$\Gamma$ (that is, $\cells(D'\setminus D'')\models\Gamma$). We assume that for every attribute $A_j$ of $\signature$, the cells $c$ in $\cells(D'')$ are such that $E'(c)\in\{v_1,\dots,v_{r-1}\}$, while for every cell $c'\in\cells(D'\setminus D'')$ it holds that $E'(c')=v_r$. In this case, $V^{D''}_{r-1}$ represent the minimal cost for the prefix $D''$, and to that cost we add the cost of changing the values of all the cells in the suffix to $v_r$. By checking that the suffix of $D''$ w.r.t.~$D'$ is consistent w.r.t.~$\Gamma$, we ensure that the set of cells that we associate with the value $v_r$ satisfies the constraint (i.e.,~$p_{E'}(v_r)\models\Gamma$). Then, $V^{D''}_{r-1}$ is responsible for checking that the cells associates with the values $v_1,\dots,v_{r-1}$ are also consistent w.r.t.~$\Gamma$ (that is, $p_{E'}(v_j)\models\Gamma$ for every $j\in\{1,\dots,r-1\}$).
   
   
   %Note that in this case, we obtain an $S_{\signature}^{i_1,\dots,i_k}$-repair $E'$ of $D$ if and only if all the cells $(\ell,A_j)$ with $E'[\ell,A_j]\in v_r$ jointly satisfy $\Gamma$ (that is, $E'$ is also an $S^{i_1'\rightarrow i_1,\dots,i_k'\rightarrow i_k}_\signature$-repair of $D$). %Otherwise, we are in the third case, where the cost is $\infty$.
    
      This completes the description of the algorithm. Its correctness is based on the following simple lemma, which arises as a direct consequence of the aforementioned two observations (regarding the consistency and ordering of cells in a repair).

      \begin{lemma}
          Let $D'$ be a prefix of $D$. There exists an optimal repair $E'$ of $(M,d,D')$ in $\{v_1,\dots,v_r\}$, a prefix $D''$ of $D'$, and an optimal repair $E''$ of $D''$ in $\{v_1,\dots,v_{r-1}\}$ such that:
          \begin{itemize}
              \item $E'(c)=E''(c)$ for all $c\in\cells(D'')$, and
              \item $E'(c')=v_r$ for all $c'\in (\cells(D')\setminus\cells(D''))$.
          \end{itemize}
      \end{lemma}
      Observe that $\cells(D')\setminus\cells(D'')$ contains all the cells in the suffix of $D''$ w.r.t.~$D'$.
      
      Regarding the computational complexity, we can compute each value $V^{D'}_r$ in polynomial time, since, as aforementioned, we can compute the set of all prefixes of $D'$ in polynomial time. Moreover, it is rather straightforward that we can compute the summation in polynomial time, and also verify the condition that $\cells(D'\setminus D'')\models\Gamma$. Finally,
    there are polynomially many values $V^{D'}_r$ that we need to compute. Therefore, we conclude that the algorithm runs in polynomial time in $|D|$.
\end{proof}



==> repair-cost-old.tex <==
\subsection{Intervention Cost}
There are various ways of measuring the quality of a repair. The typical way of doing this is by measuring the \e{amount of intervention} involved in the transformation of the inconsistent database $D$ into the repair $E$. Here, we measure this intervention using the distance function $d$. More formally, we use a function $\kappa(\cdot,\cdot,\cdot)\in\reals_{\geq 0}$ that measures
the intervention cost:
$\kappa(D,E,d)$ states the extent to which $E$ differs from $D$ with respect to the distance $d$. 

%This work studies the case where  $\kappa$ is defined in various ways via the metric $(\vals,\Delta)$. 

\begin{definition}
Let $(M,d,D)$ be an inconsistent metric database, and let $E$ be a repair. Let $(c_1,\dots,c_m)$ be an ordering of $\cells(D)$ by some arbitrary predefined order over $\cells$. We denote by $d(D,E)$  the sequence of pointwise distances between the cells of $D$ and $E$:
$$d(D,E)\defeq \Big(d\big(D(c_1),E(c_1)\big),\dots,d\big(D(c_m),E(c_m)\big)\Big).\hfill\qed$$
\end{definition}

Note that the vector $d(D,E)$ consists of only nonnegative numbers. Moreover, in every position, it has a nonzero number if and only if $D$ and $E$ have different values in the corresponding cell; in this case, we will say that the corresponding cell is \e{updated} (in the formation of $E$ from $D$).

We can now define several cost functions for repairs. Let $(M,d,D)$ be an inconsistent metric database, and $E$ a repair. Let
$d(D,E)=(\delta_1,\dots,\delta_m)$.
\begin{itemize}
\item The intervention cost
$\costnum$ counts the number of value updates (regardless of the extent of each update): $$\costnum(D,E,d)\defeq\norm{d(D,E)}{0}=|
\set{i\mid \delta_i>0}|.$$ 
\item The intervention cost
$\costmax$ measures the \e{tolerance} of the repair, which is the maximal extent by which any value is updated:
$$\costmax(D,E,d)\defeq\norm{d(D,E)}{\infty}=
\max_i \set{\delta_i}.$$ 
\item The intervention cost 
$\costsum$ is the sum of all update distances:
$$\costsum(D,E,d)\defeq\norm{d(D,E)}{1}=
\sum_{i=1}^m \delta_i.$$ 
\end{itemize}

(Note that $\norm{\cdot}{\ell}$ is a metric for $\ell=1$ and $\ell=\infty$, but not for $\ell=0$, where absolute homogeneity is violated.)

\subsection{Optimization Problem}
Let $(\signature,\Gamma)$ be a schema, $\kappa$ a cost function, and
$(M,d,D)$ an inconsistent metric database. 
\begin{itemize}
\item A repair $E$ is \e{optimal on $\kappa$} if $\kappa(D,E,d)$ is minimal across all repairs $E'$; 
\item A repair $E$ is \e{$\alpha$-optimal on $\kappa$}, for $\alpha\geq 1$, if $\kappa(D,E,d)\leq\alpha\cdot\kappa(D,E',d)$ for all repairs $E'$. 
\item For a number $\tau\geq 0$, a \e{$(\kappa\leq\tau)$-repair} is a repair $E$ such that $\kappa(D,E,d)\leq\tau$.
\end{itemize}


%\subsubsection{Computational Problem}
In the computational problems that we study, we assume a fixed schema  $(\signature,\Gamma)$ where $\signature=(A_1,\dots,A_q)$, and a fixed cost function $\kappa$. Note that $\Gamma$ can be infinite, but we assume that membership of a sequence $(i_1,\dots,i_q)$ in $\Gamma$ can be tested in polynomial time in $i_1+\dots+i_q$. 

With the above fixed, we will study the following optimization problem:
given an inconsistent metric database
$(M,d,D)$, find a repair that is optimal on $\kappa$ (or an $\alpha$-approximation thereof). Note that we assume that $M$ is finite, and given as part of the input along with the distance function $d$ and the database $D$. (We later revisit the assumption that $M$ is finite, in a different setup.)

